The Importance of Suppressing Domain Style in Authorship Analysis

The prerequisite of many approaches to authorship analysis is a representation of writing style. But despite decades of research, it still remains unclear to what extent commonly used and widely accepted representations like character trigram frequencies actually represent an author's writing style, in contrast to more domain-specific style components or even topic. We address this shortcoming for the first time in a novel experimental setup of fixed authors but swapped domains between training and testing. With this setup, we reveal that approaches using character trigram features are highly susceptible to favor domain information when applied without attention to domains, suffering drops of up to 55.4 percentage points in classification accuracy under domain swapping. We further propose a new remedy based on domain-adversarial learning and compare it to ones from the literature based on heuristic rules. Both can work well, reducing accuracy losses under domain swapping to 3.6% and 3.9%, respectively.

==> domain-style-appendices.tex <==
\appendix

\begin{center}
\Large
{\bf Supplementary Material}

\medskip
\normalsize
for ``Adversarial Training for Domain-Invariant Writing Style Representations''

\medskip
\small
(the Appendix will be added to the paper on publication)
\end{center}


\section{Data}

From March 21 to July 2nd 2018, we downloaded every single story from fanfiction.net that was available at the time (latest available story id: 12~987~600). Some stories consists of several chapters, and for each chapter, there is a corresponding HTML file. In total, we downloaded 26,424,126 single HTML files. These had to be filtered first, because some files turned out to contain only error messages saying that the particular chapter was not available any longer. Moreover, we decided to exclude stories from the ``Crossover'' and ``Misc'' categories. Crossovers are fanfictions whose plot is connected with more than one fandom and therefore has more than just one topic label. The Misc category happens to also include crossovers, which is why they were filtered out as well. After this filtering step, we still had 24,390,714 HTML files available, corresponding to 5,800,292 usable stories in 44 languages from 1,400,958 authors writing in 10,328 different fandoms (= topics). Additionally, the HTML files include meta information about genre (e.g., ``Romance''), number of reviews, number of times favourited by another user, etc. We parsed the text using the BeautifulSoup 4 package for Python. Since our goal was to extract a ``pure'' representation of each author's writing style, we tried to remove any artefactual traces that a model could use to overfit on author. First, in-text headlines (denoted by \lstinline|<h1>| and \lstinline|<h2>| html tags) were removed. This was done since many authors include own chapter or subchapter headlines in their stories. Second, centered paragraphs were removed, as they were found to frequently include text that is neither relevant to the story nor part of it, such as acknowledgements. The same applies to paragraphs written fully in bold or underlined text. Then, the first paragraph or the first five percent of the text, whatever is more, was removed. The text was always cut at the end of a sentence. The same procedure was applied to the last paragraph / the last five percent of the text. This was done because we noticed that the first and last parts of a chapter often contain information that are not part of the actual stories (e.g. claims of authorship and / or copyright).

\input{table-corpus-statistics}

Furthermore, strings containing repeating character patterns ("$\sim$+$\sim$+$\sim$+$\sim$+$\sim$") often used for demarcation were deleted, as well as * signs. The latter were sometimes used by authors at the start of each of their sentences. It was also made sure to attain a unified quotation string, all quotation characters (backticks, forwardticks, double quotes) were replaced by a single quote sign. Finally, paragraphs that begin with the word "disclaimer" or "dedication" and are followed by a colon were removed. We performed this text cleaning with much attention to detail and according to the best of our knowledge and belief. Given the vast nature of the corpus, we certainly could not get rid of every single artefact, but we may assume the rest of noise to be negligible.

%%% ADDITION.
% \input{table-author-intersection}

\section{Models}

Where we do not state anything else, we use the standard parameters of tensorflow 1.12.0~\cite{abadi:2016} and scikit-learn 0.20~\cite{scikit-learn}.

\subsection{SVM, Random Forest and Na\"ive Bayes}

SVM, Random Forest and Na\"ive Bayes were trained with scikit-learn with random search hyperparameter tuning including 3-fold cross validation. For the SVM, optimized parameters included kernel, gamma, C, and degree. 60 different parameter combinations are tested with an increased cache size of 2GB and stopping of the optimization after maximal 10000 iterations. For the Random Forest, we optimized n\_estimators, max\_depth, min\_samples\_split, max\_features, bootstrap, and criterion. Finally, for Naive Bayes the optimized parameters included alpha and fit\_prior.

\subsubsection{Neural Network Trained on 2 Authors}

LSTM layer with 256 units - 2x fully connected layer with 64 neurons and ReLU activation function - [Author prediction: 1x fully connected layer with 64 neurons and ReLU activation function | Fandom prediction: 1x fully connected layer with 64 neurons and ReLU activation function]

Dropout of 50\% applied on fully connected layer of author prediction and fandom prediction, Adam optimizer with learning rate $10^{-5}$, batch normalization, mini-batch size 400 and random seed 1.

\subsubsection{Neural Network Trained on 10 Authors}

LSTM layer with 256 units - 2x fully connected layer with 64 neurons and ReLU activation function - [Author prediction: 1x fully connected layer with 64 neurons and ReLU activation function | Fandom prediction: 1x fully connected layer with 64 neurons and ReLU activation function]

Dropout of 50\% applied on fully connected layer of author prediction and fandom prediction, Adam optimizer with learning rate $10^{-3}$, batch normalization, mini-batch size 400 and random seed 1.



==> domain-style-lit.tex <==
\begin{thebibliography}{}

\bibitem[\protect\citeauthoryear{Abadi \bgroup et al\mbox.\egroup
  }{2016}]{abadi:2016}
Abadi, M.; Barham, P.; Chen, J.; Chen, Z.; et al.
\newblock 2016.
\newblock Tensorflow: A system for large-scale machine learning.
\newblock In {\em Proc. of OSDI~2016}, 265--283.

\bibitem[\protect\citeauthoryear{Baldi and
  Sadowski}{2013}]{baldi:2013}
Baldi, P., and Sadowski, P.~J.
\newblock 2013.
\newblock Understanding dropout.
\newblock In {\em Proc. of NIPS~2013}, 2814--2822.

\bibitem[\protect\citeauthoryear{Bevendorff \bgroup et al\mbox.\egroup
  }{2019}]{stein:2019l}
Bevendorff, J.; Potthast, M.; Hagen, M.; and Stein, B.
\newblock 2019.
\newblock Heuristic authorship obfuscation.
\newblock In {\em Proc. of ACL~2019}, 1098--1108.

\bibitem[\protect\citeauthoryear{Bogdanova and
  Lazaridou}{2014}]{bogdanova:2014}
Bogdanova, D., and Lazaridou, A.
\newblock 2014.
\newblock Cross-language authorship attribution.
\newblock In {\em Proc. of LREC~2014}, 2015--2020.

\bibitem[\protect\citeauthoryear{Boumber, Zhang, and
  Mukherjee}{2018}]{boumber:2018}
Boumber, D.; Zhang, Y.; and Mukherjee, A.
\newblock 2018.
\newblock Experiments with convolutional neural networks for multi-label
  authorship attribution.
\newblock In {\em Proc. of LREC~2018}.

\bibitem[\protect\citeauthoryear{Dai \bgroup et al\mbox.\egroup
  }{2019}]{dai:2019}
Dai, N.; Liang, J.; Qiu, X.; and Huang, X.
\newblock 2019.
\newblock Style transformer: Unpaired text style transfer without
  disentangled latent representation.
\newblock {\em arXiv:1905.05621}.

\bibitem[\protect\citeauthoryear{{Ding} \bgroup et al\mbox.\egroup
  }{2019}]{ding:2019}
Ding, S.; Fung, B.; Iqbal, F.; and Cheung, W.
\newblock 2019.
\newblock Learning stylometric representations for authorship analysis.
\newblock {\em IEEE Transactions on Cybernetics} 49(1):107--121.

\bibitem[\protect\citeauthoryear{Emmery, {Manjavacas Arevalo}, and
  Chrupa{\l}a}{2018}]{emmery:2018}
Emmery, C.; {Manjavacas Arevalo}, E.; and Chrupa{\l}a, G.
\newblock 2018.
\newblock {Style Obfuscation by Invariance}.
\newblock In {\em Proc. of Coling 2018},  984--996.

\bibitem[\protect\citeauthoryear{Francis}{1965}]{francis:1965}
Francis, W.
\newblock 1965.
\newblock A standard corpus of edited present-day American English.
\newblock {\em College English} 26(4):267--273.

\bibitem[\protect\citeauthoryear{Fu \bgroup et al\mbox.\egroup
  }{2018}]{fu:2017}
Fu, Z.; Tan, X.; Peng, N.; Zhao, D.; and Yan, R.
\newblock 2018.
\newblock Style transfer in text: Exploration and evaluation.
\newblock {\em Proc. of AAAI~2018}, 663--670.

\bibitem[\protect\citeauthoryear{Ganin \bgroup et al\mbox.\egroup
  }{2016}]{ganin:2016}
Ganin, Y.; Ustinova, E.; Ajakan, H.; Germain, P.; et al.
\newblock 2016.
\newblock Domain-adversarial training of neural networks.
\newblock {\em Journal of Machine Learning Research} 17(1):2096--2030.

\bibitem[\protect\citeauthoryear{{Gatys}, {Ecker}, and
  {Bethge}}{2016}]{gatys:2016}
Gatys, L.; Ecker, A.; and Bethge, M.
\newblock 2016.
\newblock Image style transfer using convolutional neural networks.
\newblock In {\em Proc. of CVPR~2016}, 2414--2423.

\bibitem[\protect\citeauthoryear{Glorot and
  Bengio}{2010}]{glorot:2010}
Glorot, X., and Bengio, Y.
\newblock 2010.
\newblock Understanding the difficulty of training deep feedforward neural
  networks.
\newblock In {\em Proc. of \mbox{AISTATS}~2010}, 249--256.

\bibitem[\protect\citeauthoryear{Goodfellow, Bengio, and
  Courville}{2016}]{goodfellow:2016}
Goodfellow, I.; Bengio, Y.; and Courville, A.
\newblock 2016.
\newblock {\em Deep Learning}.
\newblock MIT Press.

\bibitem[\protect\citeauthoryear{Grieve}{2007}]{grieve:2007}
Grieve, J.
\newblock 2007.
\newblock Quantitative authorship attribution: An evaluation of
  techniques.
\newblock {\em Literary and Linguistic Computing} 22(3):251--270.

\bibitem[\protect\citeauthoryear{Hassan \bgroup et al\mbox.\egroup
  }{2017}]{hassan:2017}
Hassan, S.-U.; Imran, M.; Iftikhar, T.; Safder, I.; and Shabbir, M.
\newblock 2017.
\newblock Deep stylometry and lexical {\&} syntactic features based author
  attribution on plos digital repository.
\newblock In {\em Proc. of ICADL~2017}, 119--127.

\bibitem[\protect\citeauthoryear{{He} \bgroup et al\mbox.\egroup
  }{2015}]{he:2015}
He, K.; Zhang, X.; Ren, S.; and Sun, J.
\newblock 2015.
\newblock Delving deep into rectifiers: Surpassing human-level performance on
  ImageNet classification.
\newblock In {\em Proc. of ICCV~2015}, 1026--1034.

\bibitem[\protect\citeauthoryear{Hochreiter and
  Schmidhuber}{1997}]{hochreiter:1997}
Hochreiter, S., and Schmidhuber, J.
\newblock 1997.
\newblock Long short-term memory.
\newblock {\em Neural Computation} 9(8):1735--1780.

\bibitem[\protect\citeauthoryear{Hu \bgroup et al\mbox.\egroup
  }{2017}]{hu:2017}
Hu, Z.; Yang, Z.; Liang, X.; Salakhutdinov, R.; and Xing, E.~P.
\newblock 2017.
\newblock Toward controlled generation of text.
\newblock In {\em Proc. of ICML~2017}, 1587--1596.

\bibitem[\protect\citeauthoryear{Ioffe and
  Szegedy}{2015}]{ioffe:2015}
Ioffe, S., and Szegedy, C.
\newblock 2015.
\newblock Batch normalization: Accelerating deep network training by reducing
  internal covariate shift.
\newblock In {\em Proc. of ICML~2015}, 448--456.

\bibitem[\protect\citeauthoryear{Jhamtani \bgroup et al\mbox.\egroup
  }{2017}]{jhamtani:2017}
Jhamtani, H.; Gangal, V.; Hovy, E.; and Nyberg, E.
\newblock 2017.
\newblock Shakespearizing modern language using copy-enriched sequence to
  sequence models.
\newblock In {\em Proc. of Style Variation Workshop @ EMNLP~2017}, 10--19.

\bibitem[\protect\citeauthoryear{Jin \bgroup et al\mbox.\egroup
  }{2019}]{jin:2019}
Jin, Z.; Jin, D.; Mueller, J.; Matthews, N.; and Santus, E.
\newblock 2019.
\newblock Unsupervised text style transfer via iterative matching and
  translation.
\newblock {\em arXiv:1901.11333}.

\bibitem[\protect\citeauthoryear{Kabbara and
  Cheung}{2016}]{kabbara:2016}
Kabbara, J., and Cheung, J. C.~K.
\newblock 2016.
\newblock Stylistic transfer in natural language generation systems using
  recurrent neural networks.
\newblock In {\em Proc. of Uphill Battles in Language Processing Workshop @ EMNLP~2016},  43--47.

\bibitem[\protect\citeauthoryear{Kestemont \bgroup et al\mbox.\egroup
  }{2018}]{kestemont:2018}
Kestemont, M.; Tschuggnall, M.; Stamatatos, E.; Daelemans, W.; et al.
\newblock 2018.
\newblock Overview of the author identification task at PAN~2018:
  Cross-domain authorship attribution and style change detection.
\newblock In {\em Working Notes of CLEF~2018},  1--25.

\bibitem[\protect\citeauthoryear{Kingma and
  Ba}{2014}]{kingma:2014}
Kingma, D.~P., and Ba, J.
\newblock 2014.
\newblock Adam: A method for stochastic optimization.
\newblock {\em arXiv:1412.6980}.

\bibitem[\protect\citeauthoryear{Koppel and Schler}{2004}]{koppel:2004}
Koppel, M., and Schler, J.
\newblock 2004.
\newblock Authorship verification as a one-class classification problem.
\newblock In {\em Proc. of ICML~2004}.

\bibitem[\protect\citeauthoryear{Koppel \bgroup et al\mbox.\egroup
  }{2006}]{koppel:2006}
Koppel, M.; Schler, J.; Argamon, S.; and Messeri, E.
\newblock 2006.
\newblock Authorship attribution with thousands of candidate authors.
\newblock In {\em Proc. of SIGIR~2006}, 659--660.

\bibitem[\protect\citeauthoryear{Maaten and
  Hinton}{2008}]{maaten:2008}
Maaten, L., and Hinton, G.
\newblock 2008.
\newblock Visualizing data using t-SNE.
\newblock {\em Journal of Machine Learning Research} 9:2579--2605.

\bibitem[\protect\citeauthoryear{Mikros}{2007}]{mikros:2007}
Mikros, G.
\newblock 2007.
\newblock Investigating topic influence in authorship attribution.
\newblock In {\em Proc. of PAN Workshop @ SIGIR~2007}.

\bibitem[\protect\citeauthoryear{Neal \bgroup et al\mbox.\egroup
  }{2017}]{neal:2018}
Neal, T.; Sundararajan, K.; Fatima, A.; Yan, Y.; et al.
\newblock 2017.
\newblock Surveying stylometry techniques and applications.
\newblock {\em ACM Computing Surveys} 50(6):86:1--86:36.

\bibitem[\protect\citeauthoryear{Overdorf and
  Greenstadt}{2016}]{overdorf:2016}
Overdorf, R., and Greenstadt, R.
\newblock 2016.
\newblock Blogs, twitter feeds, and reddit comments: Cross-domain
  authorship attribution.
\newblock {\em Proceedings on Privacy Enhancing Technologies} 2016(3):155--171.

\bibitem[\protect\citeauthoryear{Pedregosa \bgroup et al\mbox.\egroup
  }{2011}]{scikit-learn}
Pedregosa, F.; Varoquaux, G.; Gramfort, A.; Michel, V.; et al.
\newblock 2011.
\newblock Scikit-learn: Machine learning in Python.
\newblock {\em Journal of Machine Learning Research} 12:2825--2830.

\bibitem[\protect\citeauthoryear{Potthast, Hagen, and
  Stein}{2016}]{stein:2016k}
Potthast, M.; Hagen, M.; and Stein, B.
\newblock 2016.
\newblock {Author Obfuscation: Attacking the State of the Art in Authorship
  Verification}.
\newblock In {\em Working Notes of CLEF 2016}, 1--34.

\bibitem[\protect\citeauthoryear{Prabhumoye \bgroup et al\mbox.\egroup
  }{2018}]{prabhumoye:2018}
Prabhumoye, S.; Tsvetkov, Y.; Salakhutdinov, R.; and Black, A.
\newblock 2018.
\newblock Style transfer through back-translation.
\newblock In {\em Proc. of ACL~2018}, 866--876.

\bibitem[\protect\citeauthoryear{Ruder, Ghaffari, and
  Breslin}{2016}]{ruder:2016}
Ruder, S.; Ghaffari, P.; and Breslin, J.
\newblock 2016.
\newblock Character-level and multi-channel convolutional neural networks for
  large-scale authorship attribution.
\newblock {\em arXiv:1609.06686}.

\bibitem[\protect\citeauthoryear{Shen \bgroup et al\mbox.\egroup
  }{2017}]{shen:2017}
Shen, T.; Lei, T.; Barzilay, R.; and Jaakkola, T.
\newblock 2017.
\newblock Style transfer from non-parallel text by cross-alignment.
\newblock In {\em Proc. of NIPS~2017}, 6830--6841.

\bibitem[\protect\citeauthoryear{Srivastava \bgroup et al\mbox.\egroup
  }{2014}]{srivastava:2014}
Srivastava, N.; Hinton, G.; Krizhevsky, A.; Sutskever, I.; and Salakhutdinov,
  R.
\newblock 2014.
\newblock Dropout: A simple way to prevent neural networks from overfitting.
\newblock {\em Journal of Machine Learning Research} 15:1929--1958.

\bibitem[\protect\citeauthoryear{Stamatatos}{2009}]{stamatatos:2009}
Stamatatos, E.
\newblock 2009.
\newblock A survey of modern authorship attribution methods.
\newblock {\em Journal of the American Society for Information Science and
  Technology} 60(3):538--556.

\bibitem[\protect\citeauthoryear{Stamatatos}{2013}]{stamatatos:2013}
Stamatatos, E.
\newblock 2013.
\newblock On the robustness of authorship attribution based on
  character n-gram features.
\newblock {\em Journal of Law \& Policy} 421--439.

\bibitem[\protect\citeauthoryear{Stamatatos}{2017}]{stamatatos:2017}
Stamatatos, E.
\newblock 2017.
\newblock Authorship attribution using text distortion.
\newblock In {\em Proc. of EACL~2017}, 1138--1149.

\bibitem[\protect\citeauthoryear{Zhang \bgroup et al\mbox.\egroup
  }{2018}]{zhang:2018}
Zhang, Z.; Ren, S.; Liu, S.; Wang, J.; et al.
\newblock 2018.
\newblock Style transfer as unsupervised machine translation.
\newblock {\em arXiv:1808.07894}.

\end{thebibliography}


==> figure-tsne-visualization.tex <==
\begin{figure*}[tb]%
\small%
\hspace*{-2em}%
\includegraphics[width=0.3\textwidth]{plot-two-fandoms-without-adversarial-training}%
\hspace*{-2em}%
\includegraphics[width=0.3\textwidth]{plot-two-fandoms-with-adversarial-training}%
\hspace*{-2em}%
\includegraphics[width=0.3\textwidth]{plot-ten-authors-without-adversarial-training}%
\hspace*{-2em}%
\includegraphics[width=0.3\textwidth]{plot-ten-authors-with-adversarial-training}\\[-2ex]
\null\hspace{2cm}(a)\hspace{3cm}(b)\hspace{4.5cm}(c)\hspace{3cm}(d) \\
\vspace{-3ex}%
\caption{t-SNE~\cite{maaten:2008} visualizations of the learned writing style representations with respect to two fandoms (a,b) and ten authors (c,d) without (a,c) and with (b,d) adversarial learning}%
\label{figure-tsne-visualization}%
\vspace{-2ex}%
\end{figure*}

==> table-author-intersection.tex <==
\begin{table}%
\centering%
\small%
\renewcommand{\tabcolsep}{2pt}%
\renewcommand{\arraystretch}{1}%
\begin{tabular}{@{}crrrrrr@{}}
\toprule
\bf Fandoms & 2 & 3 & 4 & 5 & 6 & 7 \\
\midrule
\bf Authors & 8099 & 850 & 131 & 36 & 3 & 1\\
\bf Stories & 55,490 & 12,972 & 2,834 & 1,206 & 228 & 231\\
\bottomrule
\end{tabular}%
\caption{Authors and stories, when greedily adding fandoms, so that all authors have written in each fandom.}%
\label{table-author-intersection}%
\vspace{-2ex}%
\end{table}


==> table-corpus-statistics.tex <==
\begin{table}[tb]%
\centering%
\small%
\renewcommand{\tabcolsep}{1pt}%
\renewcommand{\arraystretch}{1}%
\begin{tabular}{@{}l@{\kern-0.5em}r@{}r@{\ \ }rrr@{}}
\toprule
\bf Language & \bf Stories\ \ \null & \bf Fandoms & \multicolumn{3}{@{}c@{}}{\bf Text Length (Characters)} \\
\cmidrule(r@{\tabcolsep}){4-6}\cmidrule(l@{\tabcolsep}){4-6}
& & & Avg. & Std. Dev. & Max. \\
\midrule
English    & 5,098,568  & 10,012 & 53,015 & 179,701 & 216,007,457 \\
Spanish    & 320,272    & 3,101  & 66,365 & 184,807 & 16,050,508  \\
French     & 148,761    & 2,397  & 76,721 & 204,072 & 8,074,334   \\
Indonesian & 108,290    & 1,418  & 43,785 & 95,669  & 5,356,883   \\
Portuguese & 68,908     & 1,454  & 59,054 & 163,997 & 7,069,225   \\
German     & 27,227     & 987    & 80,506 & 225,056 & 10,688,021  \\
Russian    & 8,668      & 378    & 50,342 & 163,651 & 5,635,119   \\
Italian    & 3,883      & 395    & 53,526 & 154,042 & 3,600,036   \\
Hungarian  & 2,076      & 259    & 70,967 & 211,417 & 4,506,201   \\
\bottomrule
\end{tabular}%
\caption{Corpus statistics by text language}
\label{table-corpus-statistics}%
\end{table}

==> table-experiment3-schema.tex <==
%\begin{table}[!h]
%\centering
\begin{center}
\small
\setlength\tabcolsep{5pt}
\begin{tabular}{l|l:l:l:l|l:l:l:l}
        & \multicolumn{4}{c|}{normal} & \multicolumn{4}{c}{swapped} \\ \hline
authors & A     & A    & B    & B     & A    & A    & B    & B      \\
fandoms & X     & Y    & V    & W     & V    & W    & X    & Y
\end{tabular}
\end{center}
%\end{table}

